Tail Bounds on the Runtime of Categorical Compact Genetic Algorithm

The majority of theoretical analyses of evolutionary algorithms in the discrete domain focus on binary optimization algorithms, even though black-box optimization on the categorical domain has a lot of practical applications. In this paper, we consider a probabilistic model-based algorithm using the family of categorical distributions as its underlying distribution and set the sample size as two. We term this specific algorithm the categorical compact genetic algorithm (ccGA). The ccGA can be considered as an extension of the compact genetic algorithm (cGA), which is an efficient binary optimization algorithm. We theoretically analyze the dependency of the number of possible categories $K$, the number of dimensions $D$, and the learning rate $\eta$ on the runtime. We investigate the tail bound of the runtime on two typical linear functions on the categorical domain: categorical OneMax (COM) and KVal. We derive that the runtimes on COM and KVal are $O(\sqrt{D} \ln (DK) / \eta)$ and $\Theta(D \ln K/ \eta)$ with high probability, respectively. Our analysis is a generalization for that of the cGA on the binary domain.

==> macro.tex <==
% ============================================= %
% package
% ============================================= %
%\usepackage{url}
\usepackage{amssymb}
\usepackage{amsmath, amsthm}
%\usepackage{comment}
%\usepackage{bm}
%\usepackage{subcaption}
%\usepackage{remreset}
%\usepackage{cite}
\usepackage[dvipdfmx]{graphicx}
%\usepackage{setspace}
%\usepackage{subcaption}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{setspace}
\usepackage{subfig}
\usepackage{stmaryrd}
% ============================================= %
% command
% ============================================= %
% mathmatical macro
\newcommand{\argmax}{\mathop{\rm arg~max}\limits}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\N}{\mathrm{N}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\diff}{{\rm d}}

\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}


% 
\newcommand{\poly}{{\rm poly}}
\newcommand{\LIN}{\textsc{Linear}}
\newcommand{\KVAL}{f_{\,\textsc{kv}}}
\newcommand{\ONE}{f_{\,\textsc{com}}}
\newcommand{\er}{\mathcal{E}}
\newcommand{\opt}{{\rm opt}}

\newcommand*{\target}[1][true]{\ifthenelse{\boolean{#1}}{ccGA\ }{ccGA}}

\newcommand{\event}[1][t]{E^{(#1)}}
\newcommand{\bevent}[1][t]{\bar{E}^{(#1)}}

\newcommand{\param}[1][t]{\theta^{(#1)}}
\newcommand{\sample}[1][1]{x^{\langle #1 \rangle}}
\newcommand{\util}[1][1]{u^{\langle #1 \rangle}}
\newcommand{\F}[1][t]{\mathcal{F}^{(#1)}}
\newcommand{\X}[1][t]{X^{(#1)}}
\newcommand{\tX}[1][t]{\tilde{X}^{(#1)}}
\newcommand{\Y}[1][t]{Y^{(#1)}}
\newcommand{\indic}[1][E^{(t)}]{\mathbf{1}_{\{{#1}\}}}
\newcommand{\intrange}[2]{{\llbracket  #1, #2 \rrbracket}}

\newcommand{\tparam}[1][t]{\tilde{\theta}^{(#1)}}

\newcommand{\df}{d_\mathrm{f}}
\newcommand{\dfs}[1][1]{d_\mathrm{f}^{\langle #1 \rangle}}
\newcommand{\dfmin}{d_{\mathrm{f}, \mathrm{min}}}
\newcommand{\dfmax}{d_{\mathrm{f}, \mathrm{max}}}




%\newcommand{\cone}[1][1]{c_{#1}^\textsc{om}}
%\newcommand{\xione}[1][1]{\xi_{#1}^\textsc{om}}
%\newcommand{\ckv}[1][1]{c_{#1}^\textsc{kv}}
%\newcommand{\xikv}[1][1]{\xi_{#1}^\textsc{kv}}
\newcommand{\cone}[1][1]{c_{#1}}
\newcommand{\xione}[1][1]{\xi_{#1}}
\newcommand{\ckv}[1][1]{c_{#1}}
\newcommand{\xikv}[1][1]{\xi_{#1}}


% Editing Commands
% based on Niko's editing command.
%
% REQUIREMENT:
\usepackage{xcolor}
\usepackage{ifthen}
%
%------- Tool to display colored notes and changes in the draft and remove them easily
% The available commands are \del, \new, \nnew, \note, \nnote, \todo (same as \TODO).
% All commands take as optional argument the author.  The nn versions give more pronounced colors.
% Example:
%   This is\del{ an experimental version of}\note[Niko]{remark the space within the del command}
%   a \new{simple to use} LaTeX markup.\todo{improve this example}
%------- Meta-command to markup notes and changes and *remove those markups easily*
\newcommand{\markupdraft}[2]{% {#1: {color|display} command}{#2: desired color or text}
%  the next lines can be incommented, if respectively certain notes or coloring should disappear
    \ifthenelse{\equal{#1}{display}}{#2}{}%                 % display only in draft version
    \ifthenelse{\equal{#1}{color}}{\color{#2}}{}%           % colored only in draft (for \new command)
}
% ------ helper commands using \markupdraft, author is optional argument
\newcommand{\notecolored}[3][]{\markupdraft{display}{{\color{#2}\noindent[Note (#1): #3]}}}
\newcommand{\newcolored}[3][]{{\markupdraft{color}{#2}#3}%  % kept in the final print
    \ifthenelse{\equal{#1}{}}{}{\markupdraft{display}{{\color{yellow!70!black}[#1]}}}}
% ------ end user markupdraft-commands, optional argument is the author:
\newcommand{\del}[2][]{{\markupdraft{display}{{\color{orange}[removed: ``#2''[#1]]}}}} % (to be) removed
\newcommand{\new}[2][]{\newcolored[#1]{blue}{#2}}%  % kept in the final print
\newcommand{\nnew}[2][]{\newcolored[#1]{red}{#2}}%  % kept in the final print
\newcommand{\note}[2][]{\notecolored[#1]{green}{#2}}
\newcommand{\nnote}[2][]{\notecolored[#1]{magenta}{#2}}   % note with Anne's preferred default color
\newcommand{\future}[2][]{{\markupdraft{display
}{{\color{magenta}[[future:]#2[#1]]}}}}  % don't keep in current final print, but for the future
\newcommand{\calc}[2][]{{\markupdraft{display}{{\color{purple} Derived as follows: {#2}[#1]}}}} % for describe the detail in derivations.
\newcommand{\TODO}[2][]{\markupdraft{display}{{\color{red}~\\\noindent== TODO: #2 {\color{yellow}(#1)} ==\\}}}
\newcommand{\todo}[2][]{\markupdraft{display}{{\color{red}\noindent++TODO: #2 {\color{yellow}(#1)}++}}}
% ------ Final version
\renewcommand{\del}[2]{}  % make removed sentences invisible
%\renewcommand{\calc}[2]{}  % make removed sentences invisible
% \renewcommand{\markupdraft}[2]{}  % remove all todo's, notes and coloring of changes
% like for the final version
% ------ Usage
\newcommand{\yohe}[1]{\note[Youhei]{\color{cyan} #1}}
\newcommand{\shin}[1]{\note[Shinichi]{\color{magenta} #1}}
\newcommand{\kento}[1]{\note[Kento]{\color{brown} #1}}
\newcommand{\ryoki}[1]{\note[Ryoki]{\color{purple} #1}}
\newcommand{\rev}[1]{\textcolor{red}{#1}}
\providecommand{\ya}[1]{\textcolor{red}{Comment: #1}}
\providecommand{\gap}[1]{\textcolor{blue}{Flaw?: #1}}

\renewcommand{\paragraph}[1]{\textbf{#1}\ }

\usepackage[colorlinks=false,pdfborder={0 0 0}]{hyperref}
\usepackage{cleveref}
